Theoretical and Numerical Investigation of Nonlinear Thermoacoustic, Acoustic, and Detonation Waves

We begin with the theoretical study of spectral energy cascade due to the propagation of high amplitude sound in the absence of thermal sources. To this end, a first-principles-based system of governing equations, correct up to second order in perturbation variables is derived. The exact energy corollary of such second-order system of equations is then formulated and used to elucidate the spectral energy dynamics of nonlinear acoustic waves. We then extend this analysis to thermoacoustically unstable waves -- i.e. amplified as a result of thermoacoustic instability. We drive such instability up until the generation of shock waves. We further study the nonlinear wave propagation in geometrically complex case of waves induced by the spark plasma between the electrodes. This case adds the geometrical complexity of a curved, three-dimensional shock, yielding vorticity production due to baroclinic torque. Finally, detonation waves are simulated by using a low-order approach, in a periodic setup subjected to high pressure inlet and exhaust of combustible gaseous mixture. An order adaptive fully compressible and unstructured Navier Stokes solver is currently under development to enable higher fidelity studies of both the spark plasma and detonation wave problem in the future.

==> output <==
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019/Debian) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./thesis.tex
LaTeX2e <2020-02-02> patch level 2
L3 programming layer <2020-02-14> (./puthesis.cls
Document Class: puthesis 2017/03/06 Purdue thesis class, version 1.9.23
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texlive/texmf-dist/tex/latex/endnotes/endnotes.sty)
(./pulongtable.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/rotating.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/pdftex.def))))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texlive/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/share/texlive/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/base/report.cls
Document Class: report 2019/12/20 v1.4l Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size12.clo))
(/usr/share/texlive/texmf-dist/tex/latex/cite/cite.sty))
(/usr/share/texlive/texmf-dist/tex/latex/natbib/natbib.sty

Package natbib Warning: The `cite' package should not be used
(natbib)                with natbib. Use option `sort' instead.

) (/usr/share/texlive/texmf-dist/tex/latex/epstopdf-pkg/epstopdf.sty
(/usr/share/texlive/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/share/texlive/texmf-dist/tex/latex/grfext/grfext.sty
(/usr/share/texlive/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty))
(/usr/share/texlive/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/share/texlive/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/share/texlive/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty))
(/usr/share/texlive/texmf-dist/tex/latex/pdftexcmds/pdftexcmds.sty)
(/usr/share/texlive/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg)))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/epsfig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/share/texlive/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/share/texlive/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/share/texlive/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texlive/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/share/texlive/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/share/texlive/texmf-dist/tex/generic/atbegshi/atbegshi.sty))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/atveryend/atveryend.sty)
(/usr/share/texlive/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty
(/usr/share/texlive/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/cancel/cancel.sty)
(/usr/share/texlive/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/array.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/pbox/pbox.sty
(/usr/share/texlive/texmf-dist/tex/latex/tools/calc.sty))
(/usr/share/texlive/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-lists.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
(/usr/share/texlive/texmf-dist/tex/latex/ms/everyshi.sty))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.code.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.de
f)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.
tex)) (/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonomet
ric.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.cod
e.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerari
thmetics.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.
code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformation
s.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.t
ex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex))
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65
.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18
.sty)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibrarytopaths.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.geometric.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshape
s.geometric.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.misc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshape
s.misc.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.symbols.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshape
s.symbols.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.arrows.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshape
s.arrows.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.callouts.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshape
s.callouts.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibraryshapes.multipart.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshape
s.multipart.code.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/jknapltx/mathrsfs.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/setspace/setspace.sty) (./macros.tex
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/footmisc/footmisc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/scalerel/scalerel.sty
(/usr/share/texlive/texmf-dist/tex/latex/etoolbox/etoolbox.sty))
(/usr/share/texlive/texmf-dist/tex/latex/stackengine/stackengine.sty
(/usr/share/texlive/texmf-dist/tex/generic/listofitems/listofitems.sty
(/usr/share/texlive/texmf-dist/tex/generic/listofitems/listofitems.tex))))
(/usr/share/texlive/texmf-dist/tex/latex/l3backend/l3backend-pdfmode.def)
No file thesis.aux.
(/usr/share/texlive/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texlive/texmf-dist/tex/latex/notoccite/notoccite.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/share/texlive/texmf-dist/tex/generic/gettitlestring/gettitlestring.sty))
(./thesis.out) (./thesis.out) ABD: EveryShipout initializing macros [1{/var/lib
/texmf/fonts/map/pdftex/updmap/pdftex.map}] [2] [3]

Package hyperref Warning: old toc file detected, not used; run LaTeX again.

[4]

Package hyperref Warning: old lot file detected, not used; run LaTeX again.

[5]

Package hyperref Warning: old lof file detected, not used; run LaTeX again.

[6] (/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/jknapltx/ursfs.fd) [7] [8]
Chapter 1.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 376.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 1 undefined on inp
ut line 391.


Package natbib Warning: Citation `Lighthill_JSV_1978' on page 1 undefined on in
put line 391.


Package natbib Warning: Citation `Whitham2011' on page 1 undefined on input lin
e 391.


Package natbib Warning: Citation `ScaloLH_JFM_2015' on page 1 undefined on inpu
t line 391.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 1 undefined on inpu
t line 391.


Package natbib Warning: Citation `Culik_AGARD_2006' on page 1 undefined on inpu
t line 391.


Package natbib Warning: Citation `Mcmanus1993review' on page 1 undefined on inp
ut line 391.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 1 undefined on in
put line 391.


Package natbib Warning: Citation `PoinsotV_numComb_2011' on page 1 undefined on
 input line 391.


Package natbib Warning: Citation `AblowitzClarkson1991' on page 1 undefined on 
input line 391.


Package natbib Warning: Citation `Gurbatov2012' on page 1 undefined on input li
ne 391.


Package natbib Warning: Citation `Nazarov2015' on page 1 undefined on input lin
e 391.


Package natbib Warning: Citation `Whitham2011' on page 1 undefined on input lin
e 391.


Package natbib Warning: Citation `Lighthill_JSV_1978' on page 1 undefined on in
put line 391.


Package natbib Warning: Citation `Gedeon_1997_Cryocoolers' on page 1 undefined 
on input line 391.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 1 undefined on inp
ut line 391.


Package natbib Warning: Citation `Naugolnykh1998' on page 1 undefined on input 
line 391.


Package natbib Warning: Citation `Truesdell_1952_JAS' on page 1 undefined on in
put line 391.

[1]

Package natbib Warning: Citation `Chapelier_jcp_2017' on page 2 undefined on in
put line 409.


Package natbib Warning: Citation `Chapelier_jcp_2017' on page 2 undefined on in
put line 409.


LaTeX Warning: Reference `eq: IntroTrig' on page 2 undefined on input line 421.



LaTeX Warning: Reference `eq: IntroTrig' on page 2 undefined on input line 421.



LaTeX Warning: Reference `fig: Introfig1' on page 2 undefined on input line 421
.

[2 <./figures/TGV_fig.pdf>]

Package natbib Warning: Citation `kolmogorov1941a' on page 3 undefined on input
 line 438.


Package natbib Warning: Citation `kolmogorov1941b' on page 3 undefined on input
 line 438.


Package natbib Warning: Citation `kolmogorov1941c' on page 3 undefined on input
 line 438.


Package natbib Warning: Citation `pope2000turbulent' on page 3 undefined on inp
ut line 456.


Package natbib Warning: Citation `tennekes1972first' on page 3 undefined on inp
ut line 456.


Package natbib Warning: Citation `schlichting1960boundary' on page 3 undefined 
on input line 456.


LaTeX Warning: Reference `fig: Introfig2' on page 3 undefined on input line 456
.

[3]

Package natbib Warning: Citation `Rayleigh_Nature_1878' on page 4 undefined on 
input line 458.

[4 <./figures/SpectraDist.pdf>]

Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 5 undefined o
n input line 465.


Package natbib Warning: Citation `Rott_ZAMP_1969' on page 5 undefined on input 
line 465.


Package natbib Warning: Citation `Rott_ZAMP_1973' on page 5 undefined on input 
line 465.


Package natbib Warning: Citation `LinSH_JFM_2016' on page 5 undefined on input 
line 465.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 5 undefined o
n input line 465.


Package natbib Warning: Citation `BiwaEtAl_JASA_2014' on page 5 undefined on in
put line 465.


Package natbib Warning: Citation `Nazarenko_2011_WT' on page 5 undefined on inp
ut line 465.


Package natbib Warning: Citation `Zakharov_2012_WT' on page 5 undefined on inpu
t line 465.

[5]

Package natbib Warning: Citation `Truesdell_1952_JAS' on page 6 undefined on in
put line 475.


Package natbib Warning: Citation `Kevlahan_1997_JFM' on page 6 undefined on inp
ut line 475.

[6 <./figures/Slip_BaroClinic_n.png>]

Package natbib Warning: Citation `JHlee_2008' on page 7 undefined on input line
 490.


Package natbib Warning: Citation `JHlee_2008' on page 7 undefined on input line
 490.


Package natbib Warning: Citation `SHEPHERD2009' on page 7 undefined on input li
ne 490.


Package natbib Warning: Citation `Erpenbeck_PoF_1964' on page 7 undefined on in
put line 490.


Package natbib Warning: Citation `Lee_JFM_1990' on page 7 undefined on input li
ne 490.


Package natbib Warning: Citation `Sharpe_PRSA_1999' on page 7 undefined on inpu
t line 490.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 7 undefined on in
put line 497.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 7 undefined on in
put line 497.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Package natbib Warning: Citation `Wolanski_RDE_2015' on page 7 undefined on inp
ut line 500.


Package natbib Warning: Citation `WintenbergerShepherd_JPP_2006' on page 7 unde
fined on input line 500.


Package natbib Warning: Citation `Bykovskii_JPP_2006' on page 7 undefined on in
put line 500.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 7 undefined on in
put line 500.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 7 undefined on in
put line 502.

[7]

Package natbib Warning: Citation `BsinghEtAl_2019_AIAA' on page 8 undefined on 
input line 506.


Package natbib Warning: Citation `Schwer_AIAA_2010' on page 8 undefined on inpu
t line 506.


Package natbib Warning: Citation `Schwer_CandF_2011' on page 8 undefined on inp
ut line 506.

[8 <./figures/ConceptProblem.pdf>]

LaTeX Warning: Reference `fig: Vortex_INTRO' on page 9 undefined on input line 
508.

[9 <./figures/Vortex_INTRO.pdf>]
Chapter 2.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 526.


Package natbib Warning: Citation `GuptaScalo_PRE_2018' on page 10 undefined on 
input line 527.


Package natbib Warning: Citation `Lighthill_JSV_1978' on page 10 undefined on i
nput line 530.


Package natbib Warning: Citation `Gedeon_1997_Cryocoolers' on page 10 undefined
 on input line 530.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 10 undefined on in
put line 530.


Package natbib Warning: Citation `Naugolnykh1998' on page 10 undefined on input
 line 530.


Package natbib Warning: Citation `Whitham2011' on page 10 undefined on input li
ne 530.


Package natbib Warning: Citation `Gurbatov_1981_JETP' on page 10 undefined on i
nput line 530.


Package natbib Warning: Citation `Naugolnykh1998' on page 10 undefined on input
 line 530.


Package natbib Warning: Citation `Gurbatov2012' on page 10 undefined on input l
ine 530.


LaTeX Warning: Reference `sec: 1DNS' on page 10 undefined on input line 537.


LaTeX Warning: Reference `sec: 2ndOrderEntropy' on page 10 undefined on input l
ine 538.


LaTeX Warning: Reference `sec: 2ndOrderNLA' on page 10 undefined on input line 
538.

[10]

LaTeX Warning: Reference `eq: NS_eqns1' on page 11 undefined on input line 556.



LaTeX Warning: Reference `eq: NS_eqns3' on page 11 undefined on input line 556.



LaTeX Warning: Reference `sec: numerics_PRE' on page 11 undefined on input line
 556.


LaTeX Warning: Reference `sec: numerics_PRE' on page 11 undefined on input line
 565.


LaTeX Warning: Reference `tab: test_cases' on page 11 undefined on input line 5
65.


LaTeX Warning: Reference `sec: numerics_PRE' on page 11 undefined on input line
 565.


LaTeX Warning: Reference `tab: test_cases' on page 11 undefined on input line 5
65.


LaTeX Warning: Reference `sec: numerics_PRE' on page 11 undefined on input line
 571.


LaTeX Warning: Reference `eq: EntropyMach' on page 11 undefined on input line 5
71.


LaTeX Warning: Reference `eq: EntropyMax' on page 11 undefined on input line 57
1.


LaTeX Warning: Reference `sec: numerics_PRE' on page 11 undefined on input line
 571.


LaTeX Warning: Reference `eq: EntropyMach' on page 11 undefined on input line 5
71.


LaTeX Warning: Reference `eq: EntropyMax' on page 11 undefined on input line 57
1.


Package natbib Warning: Citation `Cramer_PoF_2012' on page 11 undefined on inpu
t line 574.


LaTeX Warning: Reference `fig: EntropyJumps' on page 11 undefined on input line
 574.


Package natbib Warning: Citation `LiepmannRoshko' on page 11 undefined on input
 line 574.

[11]

Package natbib Warning: Citation `Morris_JASc_1949' on page 12 undefined on inp
ut line 584.

[12 <./figures/Figure1_thesis.pdf>]

LaTeX Warning: Reference `fig: EntropyScaling' on page 13 undefined on input li
ne 595.

[13 <./figures/EntropyJumps.pdf>]

LaTeX Warning: Reference `eq: EntropyMach' on page 14 undefined on input line 5
99.


LaTeX Warning: Reference `eq: EntropyMax' on page 14 undefined on input line 59
9.


Package natbib Warning: Citation `Morris_JASc_1949' on page 14 undefined on inp
ut line 599.


LaTeX Warning: Reference `sec: numerics_PRE' on page 14 undefined on input line
 599.


Package natbib Warning: Citation `Bird_MolecularGasDynamicsBook_1994' on page 1
4 undefined on input line 599.

pdfTeX warning (ext4): destination with the same identifier (name{equation.2.2.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.613  \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.2.2.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.613  \end{align}
                   [14]

LaTeX Warning: Reference `eq: PressureMach' on page 15 undefined on input line 
620.

pdfTeX warning (ext4): destination with the same identifier (name{equation.2.2.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.626 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.2.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.626 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.2.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.626 \end{align}
                 

Package natbib Warning: Citation `Ishihara_ARFM_2009' on page 15 undefined on i
nput line 629.


Package natbib Warning: Citation `Batchelor1953theory' on page 15 undefined on 
input line 629.


Package natbib Warning: Citation `pope2000turbulent' on page 15 undefined on in
put line 629.


Package natbib Warning: Citation `monin1971statistical' on page 15 undefined on
 input line 629.


Package natbib Warning: Citation `Hosokawa_PRE_2008' on page 15 undefined on in
put line 629.


Package natbib Warning: Citation `Burattini_PRE_2006' on page 15 undefined on i
nput line 629.


LaTeX Warning: Reference `sec: ScalesAcousticCascade' on page 15 undefined on i
nput line 629.


Package natbib Warning: Citation `Whitham2011' on page 15 undefined on input li
ne 635.


LaTeX Warning: Reference `fig: EntropyScaling' on page 15 undefined on input li
ne 635.


LaTeX Warning: Reference `sec: EnergyCorollary' on page 15 undefined on input l
ine 635.


LaTeX Warning: Reference `eq: per_norm' on page 15 undefined on input line 635.



LaTeX Warning: Reference `eq: PressureMach' on page 15 undefined on input line 
635.


LaTeX Warning: Reference `sec: numerics_PRE' on page 15 undefined on input line
 635.

[15]

LaTeX Warning: Reference `eq: per_norm' on page 16 undefined on input line 637.



LaTeX Warning: Reference `eq: NS_eqns1' on page 16 undefined on input line 647.



LaTeX Warning: Reference `eq: ConstitutiveEquation' on page 16 undefined on inp
ut line 647.


LaTeX Warning: Reference `eq: NS_eqns3' on page 16 undefined on input line 653.



LaTeX Warning: Reference `eq: IdealGas' on page 16 undefined on input line 653.



LaTeX Warning: Reference `eq: per_norm' on page 16 undefined on input line 653.


[16]

LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 663.



LaTeX Warning: Reference `eq: velocity' on page 17 undefined on input line 663.



LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: velocity' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: velocity' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: velocity' on page 17 undefined on input line 668.



LaTeX Warning: Reference `sec: appedixA' on page 17 undefined on input line 668
.


LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: velocity' on page 17 undefined on input line 668.



LaTeX Warning: Reference `eq: Energy_norm' on page 17 undefined on input line 6
68.


LaTeX Warning: Reference `sec: EnergyCorollary' on page 17 undefined on input l
ine 668.


LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 670.



Package natbib Warning: Citation `Naugol1975spectrum' on page 17 undefined on i
nput line 670.


LaTeX Warning: Reference `eq: pressure' on page 17 undefined on input line 675.



LaTeX Warning: Reference `eq: velocity' on page 17 undefined on input line 675.



Package natbib Warning: Citation `Naugol1975spectrum' on page 17 undefined on i
nput line 675.


LaTeX Warning: Reference `eq: ConstitutiveEquation' on page 17 undefined on inp
ut line 675.

[17]

LaTeX Warning: Reference `eq: pressure' on page 18 undefined on input line 677.



LaTeX Warning: Reference `eq: velocity' on page 18 undefined on input line 677.



Package natbib Warning: Citation `Hamilton_NLA_1998' on page 18 undefined on in
put line 677.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 18 undefined on in
put line 681.

[18]
Chapter 3.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 686.


Package natbib Warning: Citation `GuptaScalo_PRE_2018' on page 19 undefined on 
input line 687.


Package natbib Warning: Citation `Kida_1979_JFM' on page 19 undefined on input 
line 691.


Package natbib Warning: Citation `Gurbatov_JFM_1997' on page 19 undefined on in
put line 691.


Package natbib Warning: Citation `Gurbatov1991' on page 19 undefined on input l
ine 691.


Package natbib Warning: Citation `Woyczynski_Gottingen_2006' on page 19 undefin
ed on input line 691.


Package natbib Warning: Citation `Fournier1983Burgers' on page 19 undefined on 
input line 691.


Package natbib Warning: Citation `Burgers1974nonlinear' on page 19 undefined on
 input line 691.


Package natbib Warning: Citation `batchelor1948decay' on page 19 undefined on i
nput line 692.


Package natbib Warning: Citation `batchelor1949nature' on page 19 undefined on 
input line 692.


Package natbib Warning: Citation `hinze1975turbulence' on page 19 undefined on 
input line 692.


Package natbib Warning: Citation `Ishihara_ARFM_2009' on page 19 undefined on i
nput line 692.


LaTeX Warning: Reference `eq: NS_eqns1' on page 19 undefined on input line 696.



LaTeX Warning: Reference `eq: NS_eqns3' on page 19 undefined on input line 696.


[19]

LaTeX Warning: Reference `eq: pressure' on page 20 undefined on input line 704.



LaTeX Warning: Reference `eq: velocity' on page 20 undefined on input line 704.



LaTeX Warning: Reference `fig: EnergyTime' on page 20 undefined on input line 7
04.


LaTeX Warning: Reference `eq: pressure' on page 20 undefined on input line 706.



LaTeX Warning: Reference `eq: velocity' on page 20 undefined on input line 706.



LaTeX Warning: Reference `eq: EnergyCorollary_Open' on page 20 undefined on inp
ut line 711.


LaTeX Warning: Reference `eq: LinearAcousticEnergy' on page 20 undefined on inp
ut line 724.


LaTeX Warning: Reference `fig: EnergyTime' on page 20 undefined on input line 7
24.


LaTeX Warning: Reference `eq: EnergyCorollary_Open' on page 20 undefined on inp
ut line 731.


LaTeX Warning: Reference `eq: pressure' on page 20 undefined on input line 731.


[20]

LaTeX Warning: Reference `eq: Rec1' on page 21 undefined on input line 738.


Overfull \hbox (14.49928pt too wide) detected at line 743
[]
[21 <./figures/EnergyFunction.pdf>]

LaTeX Warning: Reference `eq: Rec1' on page 22 undefined on input line 744.


LaTeX Warning: Reference `eq: Rec2' on page 22 undefined on input line 744.


LaTeX Warning: Reference `eq: energy_cons' on page 22 undefined on input line 7
63.


LaTeX Warning: Reference `eq: pressure' on page 22 undefined on input line 763.



LaTeX Warning: Reference `eq: velocity' on page 22 undefined on input line 763.



LaTeX Warning: Reference `eq: SteepeningTime' on page 22 undefined on input lin
e 771.


LaTeX Warning: Reference `eq: PcDef' on page 22 undefined on input line 771.


LaTeX Warning: Reference `tab: test_cases' on page 22 undefined on input line 7
71.


LaTeX Warning: Reference `eq: SteepeningTime' on page 22 undefined on input lin
e 771.


LaTeX Warning: Reference `eq: PcDef' on page 22 undefined on input line 771.


LaTeX Warning: Reference `tab: test_cases' on page 22 undefined on input line 7
71.


LaTeX Warning: Reference `eq: Rec1' on page 22 undefined on input line 780.


LaTeX Warning: Reference `eq: Rec2' on page 22 undefined on input line 780.

[22]

LaTeX Warning: Reference `eq: nth-term' on page 23 undefined on input line 785.


[23 <./figures/EnergyLyapunov.pdf>]

LaTeX Warning: Reference `eq: EnergyCorrection' on page 24 undefined on input l
ine 794.


Package natbib Warning: Citation `Chu1965EnergyNorm' on page 24 undefined on in
put line 795.


Package natbib Warning: Citation `myers1986exact' on page 24 undefined on input
 line 795.


LaTeX Warning: Reference `sec: appedixA' on page 24 undefined on input line 795
.


LaTeX Warning: Reference `eq: pressure' on page 24 undefined on input line 795.



LaTeX Warning: Reference `eq: velocity' on page 24 undefined on input line 795.



LaTeX Warning: Reference `eq: energy_cons' on page 24 undefined on input line 7
95.


LaTeX Warning: Reference `fig: EnergyComp' on page 24 undefined on input line 7
97.


LaTeX Warning: Reference `fig: EnergyComp' on page 24 undefined on input line 7
97.


LaTeX Warning: Reference `eq: energy_cons' on page 24 undefined on input line 7
99.

[24]

LaTeX Warning: Reference `eq: LyapunovFunction' on page 25 undefined on input l
ine 805.


LaTeX Warning: Reference `fig: EnergyTime' on page 25 undefined on input line 8
05.


LaTeX Warning: Reference `eq: pressure' on page 25 undefined on input line 805.



LaTeX Warning: Reference `eq: velocity' on page 25 undefined on input line 805.



Package natbib Warning: Citation `George2012' on page 25 undefined on input lin
e 805.


Package natbib Warning: Citation `Strogatz2018NonlinearDynamics' on page 25 und
efined on input line 805.


LaTeX Warning: Reference `eq: NS_eqns1' on page 25 undefined on input line 807.



LaTeX Warning: Reference `eq: IdealGas' on page 25 undefined on input line 807.



LaTeX Warning: Reference `eq: energy_cons' on page 25 undefined on input line 8
07.


LaTeX Warning: Reference `eq: pressure' on page 25 undefined on input line 807.



LaTeX Warning: Reference `eq: velocity' on page 25 undefined on input line 807.



Overfull \hbox (0.56703pt too wide) in paragraph at lines 807--808
[]\T1/cmr/m/n/12 Wave-front steep-en-ing en-tails cas-cade of per-tur-ba-tion e
n-ergy into higher wavenum-

LaTeX Warning: Reference `eq: NS_eqns1' on page 25 undefined on input line 815.



LaTeX Warning: Reference `eq: IdealGas' on page 25 undefined on input line 815.



LaTeX Warning: Reference `eq: Energy_norm' on page 25 undefined on input line 8
15.

[25]

LaTeX Warning: Reference `eq: DimensionlessVisc' on page 26 undefined on input 
line 824.


LaTeX Warning: Reference `eq: PcDef' on page 26 undefined on input line 824.


LaTeX Warning: Reference `eq: AcousticReynolds' on page 26 undefined on input l
ine 824.


LaTeX Warning: Reference `eq: DimensionlessVisc' on page 26 undefined on input 
line 824.


LaTeX Warning: Reference `eq: PcDef' on page 26 undefined on input line 824.


LaTeX Warning: Reference `eq: AcousticReynolds' on page 26 undefined on input l
ine 824.


LaTeX Warning: Reference `eq: PcDef' on page 26 undefined on input line 840.


LaTeX Warning: Reference `sec: ScalesAcousticCascade' on page 26 undefined on i
nput line 846.

[26]

LaTeX Warning: Reference `tab: test_cases' on page 27 undefined on input line 8
52.


LaTeX Warning: Reference `tab: test_cases' on page 27 undefined on input line 8
52.


LaTeX Warning: Reference `eq: NS_eqns1' on page 27 undefined on input line 855.



LaTeX Warning: Reference `eq: NS_eqns3' on page 27 undefined on input line 855.



Package natbib Warning: Citation `kopriva1996conservative' on page 27 undefined
 on input line 855.


Package natbib Warning: Citation `kopriva1996conservative' on page 27 undefined
 on input line 856.

[27 <./figures/AMR_tree.pdf>]

Package natbib Warning: Citation `mavriplis1994adaptive' on page 28 undefined o
n input line 858.


Package natbib Warning: Citation `mavriplis1994adaptive' on page 28 undefined o
n input line 862.


LaTeX Warning: Reference `fig: AMR' on page 28 undefined on input line 867.

[28]

LaTeX Warning: Reference `eq: per_norm' on page 29 undefined on input line 896.



LaTeX Warning: Reference `eq: FilterPU1' on page 29 undefined on input line 907
.


LaTeX Warning: Reference `sec: ScalesAcousticCascade' on page 29 undefined on i
nput line 907.


LaTeX Warning: Reference `eq: spectral_energy' on page 29 undefined on input li
ne 907.


LaTeX Warning: Reference `tab: InitialSpectra' on page 29 undefined on input li
ne 907.


LaTeX Warning: Reference `eq: FilterPU1' on page 29 undefined on input line 907
.

[29]

LaTeX Warning: Reference `eq: energy_cons' on page 30 undefined on input line 9
10.


LaTeX Warning: Reference `sec: EnergyCorollary' on page 30 undefined on input l
ine 910.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 30 undefined on i
nput line 910.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 30 undefined on i
nput line 910.


LaTeX Warning: Reference `tab: LengthScalesTable' on page 30 undefined on input
 line 910.


LaTeX Warning: Reference `sec: SpectralScaling' on page 30 undefined on input l
ine 910.


LaTeX Warning: Reference `eq: energy_cons' on page 30 undefined on input line 9
14.

[30] [31 <./figures/SpectraLengthScaleSummary_Thesis_1.png>]

LaTeX Warning: Reference `eq: SpectralEnergyRate' on page 32 undefined on input
 line 976.


LaTeX Warning: Reference `eq: spectral_conservation' on page 32 undefined on in
put line 980.

[32 <./figures/SpectraLengthScaleSummary_Thesis_2.png>]

LaTeX Warning: Reference `eq: spectral_conservation' on page 33 undefined on in
put line 1005.


LaTeX Warning: Reference `eq: SpectralDissipation' on page 33 undefined on inpu
t line 1005.


LaTeX Warning: Reference `sec: appedixB' on page 33 undefined on input line 100
5.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 33 undefined on i
nput line 1005.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 33 undefined on i
nput line 1005.


LaTeX Warning: Reference `tab: LengthScalesTable' on page 33 undefined on input
 line 1005.

[33]

LaTeX Warning: Reference `eq: SpectralFlux' on page 34 undefined on input line 
1007.


LaTeX Warning: Reference `eq: SpectralFlux' on page 34 undefined on input line 
1011.


LaTeX Warning: Reference `eq: SpectralFlux' on page 34 undefined on input line 
1011.

[34 <./figures/EnergyFluxALL.png>]

LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 35 undefined on i
nput line 1016.


LaTeX Warning: Reference `fig: EnergyFLux' on page 35 undefined on input line 1
016.


LaTeX Warning: Reference `eq: MonotonicConv' on page 35 undefined on input line
 1016.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 35 undefined on i
nput line 1016.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 35 undefined on i
nput line 1016.


LaTeX Warning: Reference `fig: EnergyFLux' on page 35 undefined on input line 1
016.

[35]

Package natbib Warning: Citation `tennekes1972first' on page 36 undefined on in
put line 1038.


Package natbib Warning: Citation `pope2000turbulent' on page 36 undefined on in
put line 1038.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 36 undefined on i
nput line 1038.


Package natbib Warning: Citation `tennekes1972first' on page 36 undefined on in
put line 1038.


Package natbib Warning: Citation `pope2000turbulent' on page 36 undefined on in
put line 1038.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 36 undefined on i
nput line 1038.

[36 <./figures/EnergyDecayALL.png>]

LaTeX Warning: Reference `eq: LyapunovFunction' on page 37 undefined on input l
ine 1040.


LaTeX Warning: Reference `eq: Microscale' on page 37 undefined on input line 10
52.


LaTeX Warning: Reference `eq: TaylorMicroscaleAssy' on page 37 undefined on inp
ut line 1063.

[37]

LaTeX Warning: Reference `fig: EnergyDecayAll' on page 38 undefined on input li
ne 1065.


LaTeX Warning: Reference `eq: IntegralLengthScale' on page 38 undefined on inpu
t line 1073.


LaTeX Warning: Reference `eq: IntegralReynoldsNumber' on page 38 undefined on i
nput line 1073.


LaTeX Warning: Reference `eq: IntegralLengthScale' on page 38 undefined on inpu
t line 1073.


LaTeX Warning: Reference `eq: IntegralReynoldsNumber' on page 38 undefined on i
nput line 1073.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 38 undefined on i
nput line 1076.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 38 undefined on i
nput line 1076.


Package natbib Warning: Citation `Gurbatov_JFM_1997' on page 38 undefined on in
put line 1082.


LaTeX Warning: Reference `eq: IntegralLengthScale' on page 38 undefined on inpu
t line 1082.

[38]

LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 39 undefined on i
nput line 1091.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 39 undefined on i
nput line 1091.


LaTeX Warning: Reference `tab: InitialSpectra' on page 39 undefined on input li
ne 1091.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 39 undefined on i
nput line 1095.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 39 undefined on i
nput line 1095.

[39 <./figures/IntegralLengthScale.pdf>]

Package natbib Warning: Citation `Gurbatov_JFM_1997' on page 40 undefined on in
put line 1101.


Package natbib Warning: Citation `Batchelor1953theory' on page 40 undefined on 
input line 1101.


Package natbib Warning: Citation `Gurbatov_JFM_1997' on page 40 undefined on in
put line 1106.


LaTeX Warning: Reference `eq: IntegralLengthScale' on page 40 undefined on inpu
t line 1106.


LaTeX Warning: Reference `eq: PLE' on page 40 undefined on input line 1106.


LaTeX Warning: Reference `eq: IntegralLengthN' on page 40 undefined on input li
ne 1115.


LaTeX Warning: Reference `eq: SpectralEnergyAssump' on page 40 undefined on inp
ut line 1120.

[40]

LaTeX Warning: Reference `eq: dEdt1' on page 41 undefined on input line 1125.


LaTeX Warning: Reference `fig: IntegralLengthScaleEvolution' on page 41 undefin
ed on input line 1126.


Package natbib Warning: Citation `Burgers1974nonlinear' on page 41 undefined on
 input line 1128.


Package natbib Warning: Citation `Kida_1979_JFM' on page 41 undefined on input 
line 1128.


LaTeX Warning: Reference `fig: IntegralLengthScaleEvolution' on page 41 undefin
ed on input line 1128.


LaTeX Warning: Reference `eq: EdotLdot' on page 41 undefined on input line 1128
.


LaTeX Warning: Reference `eq: IntegralApprox' on page 41 undefined on input lin
e 1128.


LaTeX Warning: Reference `eq: EdotLdot' on page 41 undefined on input line 1128
.


Package natbib Warning: Citation `Burgers1974nonlinear' on page 41 undefined on
 input line 1128.


Package natbib Warning: Citation `Kida_1979_JFM' on page 41 undefined on input 
line 1128.


Package natbib Warning: Citation `Gurbatov_JFM_1997' on page 41 undefined on in
put line 1128.


Package natbib Warning: Citation `Burgers1974nonlinear' on page 41 undefined on
 input line 1128.

[41]

LaTeX Warning: Reference `fig: IntegralLengthScaleEvolution' on page 42 undefin
ed on input line 1135.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 42 undefined on i
nput line 1139.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 42 undefined on i
nput line 1139.


LaTeX Warning: Reference `eq: lengthscales_centroids' on page 42 undefined on i
nput line 1144.


LaTeX Warning: Reference `eq: TaylorMicroscaleApp' on page 42 undefined on inpu
t line 1144.


Package natbib Warning: Citation `tennekes1972first' on page 42 undefined on in
put line 1145.


LaTeX Warning: Reference `eq: PcDef' on page 42 undefined on input line 1150.


LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 42 undefined on i
nput line 1150.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 42 undefined on i
nput line 1150.


LaTeX Warning: Reference `eq: TaylorMicroscaleApp' on page 42 undefined on inpu
t line 1150.


LaTeX Warning: Reference `eq: KolomogorovScale' on page 42 undefined on input l
ine 1150.


LaTeX Warning: Reference `eq: SpectralEnergyAssump' on page 42 undefined on inp
ut line 1160.


LaTeX Warning: Reference `eq: EdotLdot' on page 42 undefined on input line 1160
.

[42]

LaTeX Warning: Reference `fig: EnergyDecayAll' on page 43 undefined on input li
ne 1165.


LaTeX Warning: Reference `eq: TaylorMicroscaleApp' on page 43 undefined on inpu
t line 1165.


LaTeX Warning: Reference `eq: dEdt1' on page 43 undefined on input line 1165.


LaTeX Warning: Reference `fig: EnergyDecayAll' on page 43 undefined on input li
ne 1165.


LaTeX Warning: Reference `eq: dEdt1' on page 43 undefined on input line 1165.


LaTeX Warning: Reference `eq: KolomogorovScale' on page 43 undefined on input l
ine 1167.

[43] [44 <./figures/TravelingWaveSpectra.png>]

LaTeX Warning: Reference `eq: dEdt1' on page 45 undefined on input line 1179.


Package natbib Warning: Citation `Bec_PhyRep_2007' on page 45 undefined on inpu
t line 1184.


LaTeX Warning: Reference `eq: EnergyTimeTraveling' on page 45 undefined on inpu
t line 1187.


LaTeX Warning: Reference `fig: SpectralFlux_Traveling' on page 45 undefined on 
input line 1187.


LaTeX Warning: Reference `fig: SpectralFlux_Standing' on page 45 undefined on i
nput line 1187.


LaTeX Warning: Reference `eq: KolomogorovScale' on page 45 undefined on input l
ine 1187.


LaTeX Warning: Reference `fig: SpectralFlux_Traveling' on page 45 undefined on 
input line 1191.


LaTeX Warning: Reference `eq: SpectralForm' on page 45 undefined on input line 
1196.


LaTeX Warning: Reference `eq: SpectralForm' on page 45 undefined on input line 
1196.


LaTeX Warning: Reference `tab: test_cases' on page 45 undefined on input line 1
196.


LaTeX Warning: Reference `fig: SpectralFlux_Traveling' on page 45 undefined on 
input line 1212.


Package natbib Warning: Citation `pope2000turbulent' on page 45 undefined on in
put line 1212.


LaTeX Warning: Reference `fig: LengthScalesSummary_2' on page 45 undefined on i
nput line 1212.


LaTeX Warning: Reference `tab: test_cases' on page 45 undefined on input line 1
219.


LaTeX Warning: Reference `tab: test_cases' on page 45 undefined on input line 1
219.


LaTeX Warning: Reference `fig: EnergyDecayAll' on page 45 undefined on input li
ne 1222.


LaTeX Warning: Reference `fig: EnergyFLux' on page 45 undefined on input line 1
222.


LaTeX Warning: Reference `fig: SpectralFlux_Standing' on page 45 undefined on i
nput line 1222.


LaTeX Warning: Reference `fig: SpectralFlux_Standing' on page 45 undefined on i
nput line 1222.


LaTeX Warning: Reference `eq: KolomogorovScale' on page 45 undefined on input l
ine 1222.


LaTeX Warning: Reference `fig: SpectralFlux_Standing' on page 45 undefined on i
nput line 1222.

[45] [46 <./figures/StandingWaveSpectra.png>]

LaTeX Warning: Reference `fig: LengthScalesSummary_1' on page 47 undefined on i
nput line 1224.


Package natbib Warning: Citation `Kida_1979_JFM' on page 47 undefined on input 
line 1224.


LaTeX Warning: Reference `fig: SpectralEnergyTurbulence' on page 47 undefined o
n input line 1224.


LaTeX Warning: Reference `eq: SpectralForm' on page 47 undefined on input line 
1224.


LaTeX Warning: Reference `fig: SpectralEnergyTurbulence' on page 47 undefined o
n input line 1224.

[47] [48 <./figures/SpectralEnergyTurbulence.png>] [49]

Package natbib Warning: Citation `Burgers1974nonlinear' on page 50 undefined on
 input line 1233.

[50]
Chapter 4.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 1237.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 51 undefined on inp
ut line 1238.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 51 undefined 
on input line 1241.


Package natbib Warning: Citation `Rott_ZAMP_1969' on page 51 undefined on input
 line 1241.


Package natbib Warning: Citation `Rott_ZAMP_1973' on page 51 undefined on input
 line 1241.


Package natbib Warning: Citation `LinSH_JFM_2016' on page 51 undefined on input
 line 1241.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 51 undefined 
on input line 1241.


Package natbib Warning: Citation `BiwaEtAl_JASA_2014' on page 51 undefined on i
nput line 1241.


Package natbib Warning: Citation `Nazarenko_2011_WT' on page 51 undefined on in
put line 1241.


Package natbib Warning: Citation `Zakharov_2012_WT' on page 51 undefined on inp
ut line 1241.


Package natbib Warning: Citation `kolmogorov1941local' on page 51 undefined on 
input line 1241.

[51]

Package natbib Warning: Citation `kopriva1996conservative' on page 52 undefined
 on input line 1244.


Package natbib Warning: Citation `kopriva1996conservative2' on page 52 undefine
d on input line 1244.


Package natbib Warning: Citation `sun2007high' on page 52 undefined on input li
ne 1244.


Package natbib Warning: Citation `Jameson_JSC_2010' on page 52 undefined on inp
ut line 1244.


Package natbib Warning: Citation `persson:06' on page 52 undefined on input lin
e 1244.


Package natbib Warning: Citation `RahmanEtAl_IntJHMT_2017' on page 52 undefined
 on input line 1244.


LaTeX Warning: Reference `fig:computational_setup' on page 52 undefined on inpu
t line 1253.


LaTeX Warning: Reference `fig:computational_setup' on page 52 undefined on inpu
t line 1253.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 52 undefined 
on input line 1253.


LaTeX Warning: Reference `sec:gov_equations' on page 52 undefined on input line
 1253.


Package natbib Warning: Citation `PeneletGLB_PhysRevE_2005' on page 52 undefine
d on input line 1253.


LaTeX Warning: Reference `sec:gov_equations' on page 52 undefined on input line
 1253.


LaTeX Warning: Reference `tbl:base_state' on page 52 undefined on input line 12
54.


LaTeX Warning: Reference `sec:gov_equations' on page 52 undefined on input line
 1254.

[52]

Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 53 undefined 
on input line 1257.


LaTeX Warning: Reference `fig:optimization_lst' on page 53 undefined on input l
ine 1263.


LaTeX Warning: Reference `tbl:base_state' on page 53 undefined on input line 12
63.


LaTeX Warning: Reference `fig:optimization_lst' on page 53 undefined on input l
ine 1263.


LaTeX Warning: Reference `tbl:base_state' on page 53 undefined on input line 12
63.


Overfull \hbox (2.36983pt too wide) in paragraph at lines 1273--1273
 []|[]| 

Overfull \hbox (6.25388pt too wide) in paragraph at lines 1273--1273
 []|[]| 

Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 53 undefined 
on input line 1281.

[53] [54 <./figures/Physical_setup2.pdf>]

LaTeX Warning: Reference `fig:optimization_lst' on page 55 undefined on input l
ine 1286.


Package natbib Warning: Citation `LinSH_JFM_2016' on page 55 undefined on input
 line 1286.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 55 undefined on inp
ut line 1286.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.2.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1307 	\end{align}
                   
Overfull \hbox (4.87787pt too wide) in paragraph at lines 1322--1322
 []|\T1/cmr/m/n/12 14.51$\OT1/cmr/m/n/12 s[]$| 

Overfull \hbox (4.87787pt too wide) in paragraph at lines 1322--1323
 []|\T1/cmr/m/n/12 19.43$\OT1/cmr/m/n/12 s[]$| 

LaTeX Warning: Reference `fig:computational_setup' on page 55 undefined on inpu
t line 1325.


LaTeX Warning: Reference `fig:computational_setup' on page 55 undefined on inpu
t line 1325.


LaTeX Warning: Reference `fig:computational_setup' on page 55 undefined on inpu
t line 1325.


LaTeX Warning: Reference `fig:computational_setup' on page 55 undefined on inpu
t line 1325.


Package natbib Warning: Citation `Gedeon_Cryo_1995' on page 55 undefined on inp
ut line 1329.

[55pdfTeX warning (ext4): destination with the same identifier (name{equation.4
.2.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1330 \begin{equation}
                       ]pdfTeX warning (ext4): destination with the same identi
fier (name{equation.4.2.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1336   \begin{eqnarray}
                         pdfTeX warning (ext4): destination with the same ident
ifier (name{equation.4.2.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1336   \begin{eqnarray}
                         pdfTeX warning (ext4): destination with the same ident
ifier (name{equation.4.2.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1336   \begin{eqnarray}
                         pdfTeX warning (ext4): destination with the same ident
ifier (name{equation.4.2.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1336   \begin{eqnarray}
                          [56pdfTeX warning (ext4): destination with the same i
dentifier (name{equation.4.2.3}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1339   \end{eqnarray}
                        <./figures/Optimization.pdf>]

Package natbib Warning: Citation `kopriva1996conservative' on page 57 undefined
 on input line 1382.


Package natbib Warning: Citation `kopriva1996conservative2' on page 57 undefine
d on input line 1382.


Package natbib Warning: Citation `sun2007high' on page 57 undefined on input li
ne 1382.


Package natbib Warning: Citation `Jameson_JSC_2010' on page 57 undefined on inp
ut line 1382.


Package natbib Warning: Citation `roe1981approximate' on page 57 undefined on i
nput line 1382.


Package natbib Warning: Citation `harten1983self' on page 57 undefined on input
 line 1382.


Package natbib Warning: Citation `lodato:14b' on page 57 undefined on input lin
e 1382.


Package natbib Warning: Citation `ChapelierLJ_CF_2016' on page 57 undefined on 
input line 1382.


Package natbib Warning: Citation `persson:06' on page 57 undefined on input lin
e 1382.


Package natbib Warning: Citation `lodato:16' on page 57 undefined on input line
 1382.


Package natbib Warning: Citation `lodato2013discrete' on page 57 undefined on i
nput line 1382.


Package natbib Warning: Citation `lodato2014structural' on page 57 undefined on
 input line 1382.


Package natbib Warning: Citation `lodato:16' on page 57 undefined on input line
 1382.


Package natbib Warning: Citation `lodato:17' on page 57 undefined on input line
 1382.

[57 <./figures/mesh.pdf>]

Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 58 undefined on inp
ut line 1384.


LaTeX Warning: Reference `fig: Intro_signal' on page 58 undefined on input line
 1422.


LaTeX Warning: Reference `fig:intro_spectral' on page 58 undefined on input lin
e 1422.


LaTeX Warning: Reference `sec: Spectral energy distribution' on page 58 undefin
ed on input line 1422.


LaTeX Warning: Reference `fig:computational_setup' on page 58 undefined on inpu
t line 1427.


LaTeX Warning: Reference `fig:computational_setup' on page 58 undefined on inpu
t line 1427.


LaTeX Warning: Reference `sec: EnergyCorollary' on page 58 undefined on input l
ine 1436.


Package natbib Warning: Citation `Naugol1975spectrum' on page 58 undefined on i
nput line 1436.

[58]

LaTeX Warning: Reference `eq:energy_time' on page 59 undefined on input line 14
50.

[59 <./figures/ThermoacousticSignal_probe0014.pdf>]

LaTeX Warning: Reference `fig: Intro_signal' on page 60 undefined on input line
 1459.


LaTeX Warning: Reference `eq:dissipation_rate' on page 60 undefined on input li
ne 1465.


LaTeX Warning: Reference `eq:dissipation_rate' on page 60 undefined on input li
ne 1465.


LaTeX Warning: Reference `fig:intro_spectral' on page 60 undefined on input lin
e 1468.


LaTeX Warning: Reference `fig:intro_spectral' on page 60 undefined on input lin
e 1470.


LaTeX Warning: Reference `sec: NonlinearRegime_modeling' on page 60 undefined o
n input line 1471.


LaTeX Warning: Reference `sec: nonlinear_cascade' on page 60 undefined on input
 line 1471.

[60]

LaTeX Warning: Reference `sec: Spectral energy distribution' on page 61 undefin
ed on input line 1476.

[61 <./figures/SpectraEvo.pdf>]

Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 62 undefined on inp
ut line 1480.


Package natbib Warning: Citation `LinSH_JFM_2016' on page 62 undefined on input
 line 1484.


LaTeX Warning: Reference `sec:planar_thermoviscous_equations' on page 62 undefi
ned on input line 1484.


LaTeX Warning: Reference `sec: optimization' on page 62 undefined on input line
 1484.


LaTeX Warning: Reference `sec:Budgets' on page 62 undefined on input line 1484.



LaTeX Warning: Reference `sec: GrowthrateEffect' on page 62 undefined on input 
line 1484.

[62]

LaTeX Warning: Reference `eq: GoverningEqsLinear' on page 63 undefined on input
 line 1498.


LaTeX Warning: Reference `sec: appendixD' on page 63 undefined on input line 14
98.


LaTeX Warning: Reference `eq: 1_mass' on page 63 undefined on input line 1498.


LaTeX Warning: Reference `eq: 1_ent' on page 63 undefined on input line 1498.


LaTeX Warning: Reference `eq: 1_mom' on page 63 undefined on input line 1498.


LaTeX Warning: Reference `eq: thermoacoustic_time' on page 63 undefined on inpu
t line 1516.

[63pdfTeX warning (ext4): destination with the same identifier (name{equation.4
.4.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1520 \end{equation}
                     ]

Package natbib Warning: Citation `LinSH_JFM_2016' on page 64 undefined on input
 line 1521.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.4.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1526 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.4.4.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1526 \end{gather}
                   

LaTeX Warning: Reference `eq: thermoacoustic_time_a' on page 64 undefined on in
put line 1536.


LaTeX Warning: Reference `eq: thermoacoustic_time_b' on page 64 undefined on in
put line 1536.


LaTeX Warning: Reference `eq:energy_time' on page 64 undefined on input line 15
44.

[64]

LaTeX Warning: Reference `eq: energy' on page 65 undefined on input line 1549.


LaTeX Warning: Reference `eq:energy_spectral' on page 65 undefined on input lin
e 1554.


LaTeX Warning: Reference `eq: ModifiedRayleigh' on page 65 undefined on input l
ine 1554.


LaTeX Warning: Reference `eq: energy_density_production' on page 65 undefined o
n input line 1554.


LaTeX Warning: Reference `eq: thermoacoustic_eig' on page 65 undefined on input
 line 1554.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.4.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1559 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.4.4.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1559 \end{gather}
                   

LaTeX Warning: Reference `eq: energy_production' on page 65 undefined on input 
line 1568.


LaTeX Warning: Reference `eq: energy_production' on page 65 undefined on input 
line 1568.


LaTeX Warning: Reference `eq: energy_density_production' on page 65 undefined o
n input line 1571.


LaTeX Warning: Reference `eq: av_heat' on page 65 undefined on input line 1571.



LaTeX Warning: Reference `eq: eig_u' on page 65 undefined on input line 1571.


LaTeX Warning: Reference `eq:energy_planar' on page 65 undefined on input line 
1571.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.4.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1576 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.4.4.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1576 \end{gather}
                    [65]

LaTeX Warning: Reference `eq: budgets_production' on page 66 undefined on input
 line 1587.


LaTeX Warning: Reference `eq: budgets_production' on page 66 undefined on input
 line 1587.


LaTeX Warning: Reference `fig: ProductionTerms' on page 66 undefined on input l
ine 1590.


LaTeX Warning: Reference `fig: OptPhase' on page 66 undefined on input line 159
0.


LaTeX Warning: Reference `fig: OptPhase' on page 66 undefined on input line 159
0.


LaTeX Warning: Reference `fig: ProductionTerms' on page 66 undefined on input l
ine 1590.


LaTeX Warning: Reference `fig: OptPhase' on page 66 undefined on input line 159
0.


LaTeX Warning: Reference `tbl:base_state' on page 66 undefined on input line 15
90.

[66 <./figures/ProductionTerms.pdf>]

LaTeX Warning: Reference `eq:tau' on page 67 undefined on input line 1599.


LaTeX Warning: Reference `eq: functional_approx' on page 67 undefined on input 
line 1599.


LaTeX Warning: Reference `eq:tau' on page 67 undefined on input line 1599.


LaTeX Warning: Reference `eq: functional_approx' on page 67 undefined on input 
line 1599.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.4.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1608 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.4.4.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1608 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.4.4.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1608 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.4.4.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1608 \begin{eqnarray}
                        [67 <./figures/OptPhase.pdf>]

LaTeX Warning: Reference `fig: RayleighIndex' on page 68 undefined on input lin
e 1623.


LaTeX Warning: Reference `fig: GrowthRate' on page 68 undefined on input line 1
623.


LaTeX Warning: Reference `fig: GrowthRate' on page 68 undefined on input line 1
623.


LaTeX Warning: Reference `fig: RayleighIndex' on page 68 undefined on input lin
e 1623.

[68 <./figures/GrowthTempDres.pdf>]

LaTeX Warning: Reference `fig: GrowthRate' on page 69 undefined on input line 1
639.


LaTeX Warning: Reference `fig: RayleighIndex' on page 69 undefined on input lin
e 1640.


LaTeX Warning: Reference `eq:travelling_standing_weights' on page 69 undefined 
on input line 1640.


Package natbib Warning: Citation `BiwaEtAl_JASA_2014' on page 69 undefined on i
nput line 1644.

[69 <./figures/RayleighTempDres.pdf>]

LaTeX Warning: Reference `eq: nonlinear_P' on page 70 undefined on input line 1
646.


LaTeX Warning: Reference `sec: governing_equations' on page 70 undefined on inp
ut line 1646.


LaTeX Warning: Reference `sec: nonlinear_wave' on page 70 undefined on input li
ne 1646.


LaTeX Warning: Reference `sec: nonlinear_thermoacoustic' on page 70 undefined o
n input line 1646.


LaTeX Warning: Reference `sec: shear_heat' on page 70 undefined on input line 1
646.


Overfull \hbox (7.94577pt too wide) in paragraph at lines 1649--1652
[]\T1/cmr/m/n/12 The non-lin-ear gov-ern-ing equa-tions, cor-rect up to sec-ond
 or-der, for a two-dimensional
[70]

LaTeX Warning: Reference `eq: 2_mom' on page 71 undefined on input line 1660.


LaTeX Warning: Reference `eq: 2_ent' on page 71 undefined on input line 1660.


LaTeX Warning: Reference `eq: 2_mass' on page 71 undefined on input line 1662.


LaTeX Warning: Reference `eq: 2_ent' on page 71 undefined on input line 1662.


LaTeX Warning: Reference `eq: AcousticDynamicalSystem' on page 71 undefined on 
input line 1662.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.5.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1672 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.4.5.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1672 \end{gather}
                   

LaTeX Warning: Reference `eq: constitutive_eqn' on page 71 undefined on input l
ine 1680.


Package natbib Warning: Citation `HedbergR_JAP_2011' on page 71 undefined on in
put line 1680.


LaTeX Warning: Reference `fig: constitutive' on page 71 undefined on input line
 1680.


LaTeX Warning: Reference `eq: constitutive_eqn' on page 71 undefined on input l
ine 1680.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 71 undefined on in
put line 1681.


LaTeX Warning: Reference `eq: constitutive_eqn' on page 71 undefined on input l
ine 1681.


LaTeX Warning: Reference `eq: constitutive_eqn' on page 71 undefined on input l
ine 1681.

[71pdfTeX warning (ext4): destination with the same identifier (name{equation.4
.5.3}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1682 
       ] [72 <./figures/ConstitutivePlot.pdf>]

LaTeX Warning: Reference `fig:computational_setup' on page 73 undefined on inpu
t line 1685.


LaTeX Warning: Reference `eq: 2_mom' on page 73 undefined on input line 1685.


LaTeX Warning: Reference `eq: 2_ent' on page 73 undefined on input line 1685.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 73 undefined on in
put line 1685.


LaTeX Warning: Reference `eq: inviscid_p' on page 73 undefined on input line 16
90.


Package natbib Warning: Citation `ChuK_JFM_1958' on page 73 undefined on input 
line 1694.


Package natbib Warning: Citation `Pierce_1989' on page 73 undefined on input li
ne 1694.

[73]

LaTeX Warning: Reference `eq: shear' on page 74 undefined on input line 1710.


LaTeX Warning: Reference `eq: heat_transfer' on page 74 undefined on input line
 1710.

pdfTeX warning (ext4): destination with the same identifier (name{equation.4.5.
1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1715 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.4.5.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.1715 \end{gather}
                   

LaTeX Warning: Reference `eq: eigenfunctions_y' on page 74 undefined on input l
ine 1717.


LaTeX Warning: Reference `eq: u_modes' on page 74 undefined on input line 1723.



LaTeX Warning: Reference `eq: s_modes' on page 74 undefined on input line 1723.



LaTeX Warning: Reference `eq: 2_mom' on page 74 undefined on input line 1728.


LaTeX Warning: Reference `eq: 2_mom' on page 74 undefined on input line 1728.


Package natbib Warning: Citation `Hamilton_NLA_1998' on page 74 undefined on in
put line 1728.


LaTeX Warning: Reference `eq: eigenfunctions_y' on page 74 undefined on input l
ine 1728.

[74]

LaTeX Warning: Reference `eq: inviscid_p' on page 75 undefined on input line 17
36.


LaTeX Warning: Reference `eq: 2_mass' on page 75 undefined on input line 1736.


LaTeX Warning: Reference `eq: 2_ent' on page 75 undefined on input line 1736.


LaTeX Warning: Reference `eq: constitutive_eqn' on page 75 undefined on input l
ine 1736.


LaTeX Warning: Reference `eq: nonlinear_P' on page 75 undefined on input line 1
745.


LaTeX Warning: Reference `eq: s_modes' on page 75 undefined on input line 1745.



LaTeX Warning: Reference `eq: 2_mom' on page 75 undefined on input line 1750.


LaTeX Warning: Reference `eq: 2_ent' on page 75 undefined on input line 1750.


LaTeX Warning: Reference `eq: nonlinear_P' on page 75 undefined on input line 1
750.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 75 undefined on inp
ut line 1750.


LaTeX Warning: Reference `eq: u_modes' on page 75 undefined on input line 1750.



LaTeX Warning: Reference `eq: s_modes' on page 75 undefined on input line 1750.



LaTeX Warning: Reference `eq: nonlinear_U' on page 75 undefined on input line 1
750.


LaTeX Warning: Reference `eq: nonlinear_P' on page 75 undefined on input line 1
750.


LaTeX Warning: Reference `eq: MacrosonicThermoacousticInteraction' on page 75 u
ndefined on input line 1750.

[75]

LaTeX Warning: Reference `eq: u_modes' on page 76 undefined on input line 1757.



LaTeX Warning: Reference `eq: s_modes' on page 76 undefined on input line 1757.



LaTeX Warning: Reference `eq: u_modes' on page 76 undefined on input line 1758.



LaTeX Warning: Reference `eq: s_modes' on page 76 undefined on input line 1758.


[76]

LaTeX Warning: Reference `eq: analytical_un' on page 77 undefined on input line
 1771.


LaTeX Warning: Reference `eq: analytical_sn' on page 77 undefined on input line
 1771.


LaTeX Warning: Reference `eq: analytical_tau' on page 77 undefined on input lin
e 1776.


LaTeX Warning: Reference `eq: analytical_q' on page 77 undefined on input line 
1776.


LaTeX Warning: Reference `eq: nonlinear_U' on page 77 undefined on input line 1
776.


LaTeX Warning: Reference `eq: nonlinear_P_reduced' on page 77 undefined on inpu
t line 1776.


LaTeX Warning: Reference `eq: u_modes' on page 77 undefined on input line 1776.



LaTeX Warning: Reference `eq: s_modes' on page 77 undefined on input line 1776.



LaTeX Warning: Reference `eq: inviscid_p' on page 77 undefined on input line 17
86.


LaTeX Warning: Reference `eq: inviscid_U' on page 77 undefined on input line 17
86.


LaTeX Warning: Reference `eq: u_modes' on page 77 undefined on input line 1786.



LaTeX Warning: Reference `eq: s_modes' on page 77 undefined on input line 1786.



LaTeX Warning: Reference `eq: nonlinear_U' on page 77 undefined on input line 1
786.


LaTeX Warning: Reference `eq: nonlinear_P' on page 77 undefined on input line 1
786.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 77 undefined on inp
ut line 1786.


LaTeX Warning: Reference `eq: inviscid_p' on page 77 undefined on input line 18
10.


LaTeX Warning: Reference `eq: inviscid_U' on page 77 undefined on input line 18
10.


LaTeX Warning: Reference `eq: u_modes' on page 77 undefined on input line 1810.



LaTeX Warning: Reference `eq: s_modes' on page 77 undefined on input line 1810.



LaTeX Warning: Reference `eq: nonlinear_U' on page 77 undefined on input line 1
810.


LaTeX Warning: Reference `eq: nonlinear_P' on page 77 undefined on input line 1
810.


LaTeX Warning: Reference `eq: inviscid_p' on page 77 undefined on input line 18
10.


LaTeX Warning: Reference `eq: inviscid_U' on page 77 undefined on input line 18
10.


LaTeX Warning: Reference `eq: u_modes' on page 77 undefined on input line 1810.



LaTeX Warning: Reference `eq: s_modes' on page 77 undefined on input line 1810.



LaTeX Warning: Reference `eq: nonlinear_U' on page 77 undefined on input line 1
810.


LaTeX Warning: Reference `eq: nonlinear_P' on page 77 undefined on input line 1
810.


LaTeX Warning: `!h' float specifier changed to `!ht'.


LaTeX Warning: Reference `eq: nonlinear_P_reduced' on page 77 undefined on inpu
t line 1813.


LaTeX Warning: Reference `fig: model_signal' on page 77 undefined on input line
 1813.


LaTeX Warning: Reference `eq: nonlinear_P_reduced' on page 77 undefined on inpu
t line 1813.


LaTeX Warning: Reference `eq: MacrosonicThermoacousticInteraction' on page 77 u
ndefined on input line 1813.

[77]

LaTeX Warning: Reference `fig: model_spectra' on page 78 undefined on input lin
e 1815.


LaTeX Warning: Reference `eq:energy_spectral' on page 78 undefined on input lin
e 1815.


LaTeX Warning: Reference `sec: NonlinearRegime_modeling' on page 78 undefined o
n input line 1815.


LaTeX Warning: Reference `fig: model_signal' on page 78 undefined on input line
 1815.


LaTeX Warning: Reference `fig: model_spectra' on page 78 undefined on input lin
e 1815.

[78 <./figures/NLTA-probe.pdf>]

LaTeX Warning: Reference `eq: inviscid_p' on page 79 undefined on input line 18
17.


LaTeX Warning: Reference `eq: inviscid_U' on page 79 undefined on input line 18
17.


LaTeX Warning: Reference `eq: Burgers' on page 79 undefined on input line 1825.


[79]

LaTeX Warning: Reference `fig: model_signal' on page 80 undefined on input line
 1844.


LaTeX Warning: Reference `fig: model_signal' on page 80 undefined on input line
 1844.


LaTeX Warning: Reference `eq: CascadeFunction1' on page 80 undefined on input l
ine 1847.


LaTeX Warning: Reference `eq: CascadeFunction1' on page 80 undefined on input l
ine 1847.

[80 <./figures/SpectraEvoModel.pdf>]

LaTeX Warning: Reference `eq: overtones' on page 81 undefined on input line 185
1.


Package natbib Warning: Citation `pope2000turbulent' on page 81 undefined on in
put line 1911.


Package natbib Warning: Citation `Nazarenko_2011_WT' on page 81 undefined on in
put line 1911.

[81]

LaTeX Warning: Reference `eq:energy_time' on page 82 undefined on input line 19
15.


LaTeX Warning: Reference `eq: dissipation' on page 82 undefined on input line 1
915.


LaTeX Warning: Reference `eq: SpectralScaling' on page 82 undefined on input li
ne 1923.


LaTeX Warning: Reference `eq: SpectralScaling' on page 82 undefined on input li
ne 1923.


LaTeX Warning: Reference `eq: TotalEnergy' on page 82 undefined on input line 1
934.

[82]

LaTeX Warning: Reference `eq: SpectralScaling' on page 83 undefined on input li
ne 1938.


LaTeX Warning: Reference `fig: pressure_spectralDist' on page 83 undefined on i
nput line 1938.


LaTeX Warning: Reference `fig:intro_spectral' on page 83 undefined on input lin
e 1938.


Package natbib Warning: Citation `GuptaLS_SCITECH_2017' on page 83 undefined on
 input line 1938.


LaTeX Warning: Reference `eq: SpectralScaling' on page 83 undefined on input li
ne 1938.

[83 <./figures/SpectraDistModel.pdf>]

Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 84 undefined 
on input line 1957.

[84] [85]
Chapter 5.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 1967.


Package natbib Warning: Citation `BsinghEtAl_2019_AIAA' on page 86 undefined on
 input line 1968.


Package natbib Warning: Citation `Bsingh2018_EinF' on page 86 undefined on inpu
t line 1968.


Package natbib Warning: Citation `Corke_ARFM_2010' on page 86 undefined on inpu
t line 1972.


Package natbib Warning: Citation `Pai_PSST_2010' on page 86 undefined on input 
line 1972.


LaTeX Warning: Reference `fig:SparkElectrodes' on page 86 undefined on input li
ne 1975.


LaTeX Warning: Reference `fig:SparkElectrodesShocks' on page 86 undefined on in
put line 1988.

[86] [87 <./figures/electrodes_Spark.png> <./figures/Figure_SparkPlasmaShock.pd
f>]

Package natbib Warning: Citation `kopriva:96' on page 88 undefined on input lin
e 1991.


Package natbib Warning: Citation `sun:07' on page 88 undefined on input line 19
91.


Package natbib Warning: Citation `lodato:14b' on page 88 undefined on input lin
e 1991.


Package natbib Warning: Citation `persson:06' on page 88 undefined on input lin
e 1992.


Package natbib Warning: Citation `lodato:15' on page 88 undefined on input line
 1992.


Package natbib Warning: Citation `lodato:16' on page 88 undefined on input line
 1992.


LaTeX Warning: Reference `fig: Setup' on page 88 undefined on input line 1998.

[88 <./figures/ComputationalSetup.pdf>]

LaTeX Warning: Reference `subeq:ns1' on page 89 undefined on input line 2027.


LaTeX Warning: Reference `subeq:ns3' on page 89 undefined on input line 2027.


LaTeX Warning: Reference `fig: Setup' on page 89 undefined on input line 2027.

[89pdfTeX warning (ext4): destination with the same identifier (name{equation.5
.3.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2030 \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.5.3.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2030 \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.5.3.3}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2030 \end{align}
                  ]

LaTeX Warning: Reference `fig: FlowModeling' on page 90 undefined on input line
 2040.


LaTeX Warning: Reference `fig: InitialStagesVorticity_noslip' on page 90 undefi
ned on input line 2049.


LaTeX Warning: Reference `fig: InitialStagesVorticity_noslip' on page 90 undefi
ned on input line 2049.


LaTeX Warning: Reference `fig: InitialStagesVorticity_noslip' on page 90 undefi
ned on input line 2049.


LaTeX Warning: Reference `fig: InitialStagesVorticity_slip' on page 90 undefine
d on input line 2049.

[90]

LaTeX Warning: Reference `fig: InitialStagesVorticity_slip' on page 91 undefine
d on input line 2065.


LaTeX Warning: Reference `fig: InitialStagesBaroclinic_NoSlip' on page 91 undef
ined on input line 2074.


LaTeX Warning: Reference `fig: InitialStagesBaroclinic_Slip' on page 91 undefin
ed on input line 2074.

[91 <./figures/FlowModeling.pdf>]

LaTeX Warning: Reference `eq: baroclinic' on page 92 undefined on input line 20
80.


LaTeX Warning: Reference `fig: InitialStagesBaroclinic_NoSlip' on page 92 undef
ined on input line 2087.


LaTeX Warning: Reference `fig: InitialStagesBaroclinic_Slip' on page 92 undefin
ed on input line 2087.


LaTeX Warning: Reference `fig: InitialStagesVorticity_noslip' on page 92 undefi
ned on input line 2087.


LaTeX Warning: Reference `fig: InitialStagesVorticity_slip' on page 92 undefine
d on input line 2087.

[92 <./figures/Noslip_omega_n.pdf> <./figures/Slip_omega_n.pdf

pdfTeX warning: pdflatex (file ./figures/Slip_omega_n.pdf): PDF inclusion: mult
iple pdfs with page group included in a single page
>] [93 <./figures/NoSlip_BaroClinic_n.pdf> <./figures/Slip_BaroClinic_n.pdf

pdfTeX warning: pdflatex (file ./figures/Slip_BaroClinic_n.pdf): PDF inclusion:
 multiple pdfs with page group included in a single page
>]
Chapter 6.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2093.


Package natbib Warning: Citation `GuptaSLSS_Aviation_2018' on page 94 undefined
 on input line 2094.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 94 undefined on i
nput line 2094.


Package natbib Warning: Citation `JHlee_2008' on page 94 undefined on input lin
e 2097.


Package natbib Warning: Citation `JHlee_2008' on page 94 undefined on input lin
e 2097.


Package natbib Warning: Citation `SHEPHERD2009' on page 94 undefined on input l
ine 2097.


Package natbib Warning: Citation `Erpenbeck_PoF_1964' on page 94 undefined on i
nput line 2097.


Package natbib Warning: Citation `Lee_JFM_1990' on page 94 undefined on input l
ine 2097.


Package natbib Warning: Citation `Sharpe_PRSA_1999' on page 94 undefined on inp
ut line 2097.


Package natbib Warning: Citation `Wolanski_RDE_2015' on page 94 undefined on in
put line 2099.


Package natbib Warning: Citation `WintenbergerShepherd_JPP_2006' on page 94 und
efined on input line 2099.


Package natbib Warning: Citation `Bykovskii_JPP_2006' on page 94 undefined on i
nput line 2099.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 94 undefined on i
nput line 2099.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 94 undefined on i
nput line 2099.

[94]

Package natbib Warning: Citation `Schwer_AIAA_2010' on page 95 undefined on inp
ut line 2101.


Package natbib Warning: Citation `Schwer_CandF_2011' on page 95 undefined on in
put line 2101.


Package natbib Warning: Citation `Lietz_AIAA_2018' on page 95 undefined on inpu
t line 2101.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 95 undefined on i
nput line 2107.


LaTeX Warning: Reference `fig:DRONE_Instrumentation_Diagram' on page 95 undefin
ed on input line 2107.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 95 undefined on i
nput line 2107.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 95 undefined on i
nput line 2111.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 95 undefined on i
nput line 2111.


LaTeX Warning: Reference `fig:Test40_ChemiluminescencePCB' on page 95 undefined
 on input line 2115.


LaTeX Warning: Reference `fig:Test40_ChemiluminescencePCB' on page 95 undefined
 on input line 2115.


LaTeX Warning: Reference `fig:DRONE_Instrumentation_Diagram' on page 95 undefin
ed on input line 2115.


LaTeX Warning: Reference `fig:Test40_ChemiluminescencePCB' on page 95 undefined
 on input line 2115.

[95]

Package natbib Warning: Citation `Schwinn_CandF_2018' on page 96 undefined on i
nput line 2122.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 96 undefined on i
nput line 2122.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 96 undefined on i
nput line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 96 undefined on input 
line 2126.

[96 <./figures/DRONE_Instrumentation_Diagram.pdf> <./figures/Test40_IPrime-PPri
me+Chemiluminescence_new.pdf

pdfTeX warning: pdflatex (file ./figures/Test40_IPrime-PPrime+Chemiluminescence
_new.pdf): PDF inclusion: multiple pdfs with page group included in a single pa
ge
>]

Package natbib Warning: Citation `Schwinn_CandF_2018' on page 97 undefined on i
nput line 2131.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 97 undefined on i
nput line 2131.


LaTeX Warning: Reference `fig:Chemiluminescence' on page 97 undefined on input 
line 2135.


LaTeX Warning: Reference `fig:Test40_ChemiluminescencePCB' on page 97 undefined
 on input line 2135.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 97 undefined on i
nput line 2137.


Package natbib Warning: Citation `Jachimowski1988_Hydrogen' on page 97 undefine
d on input line 2137.


Package natbib Warning: Citation `lodato2013discrete' on page 97 undefined on i
nput line 2137.


Package natbib Warning: Citation `lodato2014structural' on page 97 undefined on
 input line 2137.


Package natbib Warning: Citation `lodato:14b' on page 97 undefined on input lin
e 2137.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 97 undefined on inp
ut line 2137.

[97 <./figures/Chemiluminescence.pdf>]

Package natbib Warning: Citation `Oran_CandF_1982' on page 98 undefined on inpu
t line 2236.


Package natbib Warning: Citation `YungsterRadha_AIAA_1996' on page 98 undefined
 on input line 2236.


Package natbib Warning: Citation `Oran_CandF_1982' on page 98 undefined on inpu
t line 2236.


Package natbib Warning: Citation `YungsterRadha_AIAA_1996' on page 98 undefined
 on input line 2236.


LaTeX Warning: Reference `fig: Validation1DDet' on page 98 undefined on input l
ine 2239.


Package natbib Warning: Citation `YungsterRadha_AIAA_1996' on page 98 undefined
 on input line 2239.


LaTeX Warning: Reference `fig: Validation1DDet' on page 98 undefined on input l
ine 2239.


LaTeX Warning: Reference `fig: Validation1DDet' on page 98 undefined on input l
ine 2239.


LaTeX Warning: Reference `fig: Validation1DDet' on page 98 undefined on input l
ine 2240.


Package natbib Warning: Citation `JHlee_2008' on page 98 undefined on input lin
e 2240.

[98]

LaTeX Warning: Reference `fig: Validation1DDet' on page 99 undefined on input l
ine 2242.


Package natbib Warning: Citation `Schwer_CandF_2011' on page 99 undefined on in
put line 2242.


Package natbib Warning: Citation `Lietz_AIAA_2018' on page 99 undefined on inpu
t line 2242.


Package natbib Warning: Citation `Fotia_AIAA_2014' on page 99 undefined on inpu
t line 2242.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 99 undefined on i
nput line 2242.

[99 <./figures/ValidationSetup.pdf>]

Package natbib Warning: Citation `goodwin2009cantera' on page 100 undefined on 
input line 2246.


LaTeX Warning: Reference `fig: LaminarFlame' on page 100 undefined on input lin
e 2246.


Package natbib Warning: Citation `vagelopoulos1994' on page 100 undefined on in
put line 2252.


Package natbib Warning: Citation `PoinsotV_numComb_2011' on page 100 undefined 
on input line 2252.


Package natbib Warning: Citation `vagelopoulos1994' on page 100 undefined on in
put line 2252.


Package natbib Warning: Citation `PoinsotV_numComb_2011' on page 100 undefined 
on input line 2252.


Package natbib Warning: Citation `Fotia_AIAA_2014' on page 100 undefined on inp
ut line 2260.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 100 undefined on 
input line 2260.


Package natbib Warning: Citation `Schwer_CandF_2011' on page 100 undefined on i
nput line 2260.


Package natbib Warning: Citation `Lietz_AIAA_2018' on page 100 undefined on inp
ut line 2260.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 100 undefined on 
input line 2266.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 100 undefined on 
input line 2266.

[100]

LaTeX Warning: Reference `fig: ConceptProblem' on page 101 undefined on input l
ine 2270.

[101 <./figures/LaminarFlame_Le1.pdf>]

LaTeX Warning: Reference `eq: 2D_governingEqs1' on page 102 undefined on input 
line 2283.


LaTeX Warning: Reference `eq: 2D_governingEqs4' on page 102 undefined on input 
line 2283.


LaTeX Warning: Reference `fig: ConceptProblem' on page 102 undefined on input l
ine 2283.


LaTeX Warning: Reference `eq: 1D_ReducedEqs1' on page 102 undefined on input li
ne 2295.


LaTeX Warning: Reference `eq: 1D_ReducedEqs4' on page 102 undefined on input li
ne 2295.


Package natbib Warning: Citation `Schwer_AIAA_2010' on page 102 undefined on in
put line 2295.

[102]

LaTeX Warning: Reference `eq: 1D_ModelEqs1' on page 103 undefined on input line
 2304.


LaTeX Warning: Reference `eq: 1D_ModelEqs4' on page 103 undefined on input line
 2304.

[103]

LaTeX Warning: Reference `eq: flowrate_nozzle' on page 104 undefined on input l
ine 2320.


LaTeX Warning: Reference `eq: rho_nozzle' on page 104 undefined on input line 2
320.


LaTeX Warning: Reference `eq: M_nozzle' on page 104 undefined on input line 232
0.

[104 <./figures/DetonationInit.pdf>]

LaTeX Warning: Reference `fig: ConceptProblem' on page 105 undefined on input l
ine 2363.


LaTeX Warning: Reference `fig: DetonationInit' on page 105 undefined on input l
ine 2363.

[105] [106 <./figures/SpatialProfiles_3P0_ws20_Labeled.pdf>]

LaTeX Warning: Reference `fig: Validation1DDet' on page 107 undefined on input 
line 2371.


LaTeX Warning: Reference `tab: TestCases' on page 107 undefined on input line 2
371.


LaTeX Warning: Reference `fig: Detonation3P0' on page 107 undefined on input li
ne 2373.


LaTeX Warning: Reference `fig: DetonationTrackHeatRelease' on page 107 undefine
d on input line 2389.

[107]

LaTeX Warning: Reference `fig: DetonationTrackHeatRelease' on page 108 undefine
d on input line 2392.


LaTeX Warning: Reference `fig: DetonationTrajectory' on page 108 undefined on i
nput line 2392.


Package natbib Warning: Citation `CEAcite' on page 108 undefined on input line 
2392.

[108 <./figures/DetonationTrackHeatRelease.pdf>]

LaTeX Warning: Reference `fig: DetonationTrackHeatRelease_ws' on page 109 undef
ined on input line 2413.

[109 <./figures/DetonationTrackTrajectory.pdf> <./figures/DetonationTrackHeatRe
lease_ws.pdf

pdfTeX warning: pdflatex (file ./figures/DetonationTrackHeatRelease_ws.pdf): PD
F inclusion: multiple pdfs with page group included in a single page
>]

Package natbib Warning: Citation `Schwinn_CandF_2018' on page 110 undefined on 
input line 2416.


Package natbib Warning: Citation `Schwinn_CandF_2018' on page 110 undefined on 
input line 2420.


Package natbib Warning: Citation `Lietz_AIAA_2018' on page 110 undefined on inp
ut line 2420.


Package natbib Warning: Citation `Schwer_AIAA_2010' on page 110 undefined on in
put line 2420.

[110] [111]
Chapter 7.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2426.


Package natbib Warning: Citation `karniadakis2005spectral' on page 112 undefine
d on input line 2431.


Package natbib Warning: Citation `Wang_2002_JCP' on page 112 undefined on input
 line 2431.


Package natbib Warning: Citation `kopriva1996conservative' on page 112 undefine
d on input line 2431.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 112 undefined on in
put line 2431.


Package natbib Warning: Citation `LodatoJ_2019_LES' on page 112 undefined on in
put line 2431.


Package natbib Warning: Citation `Zhou_2010_JCP' on page 112 undefined on input
 line 2431.


Package natbib Warning: Citation `lodato:14b' on page 112 undefined on input li
ne 2431.


Package natbib Warning: Citation `ChapelierLJ_CF_2016' on page 112 undefined on
 input line 2431.


Package natbib Warning: Citation `GuptaScalo_PRE_2018' on page 112 undefined on
 input line 2431.


Package natbib Warning: Citation `GuptaLS_JFM_2017' on page 112 undefined on in
put line 2431.


Package natbib Warning: Citation `lodato:16' on page 112 undefined on input lin
e 2431.


Package natbib Warning: Citation `lodato2013discrete' on page 112 undefined on 
input line 2431.


Package natbib Warning: Citation `LodatoJ_2019_LES' on page 112 undefined on in
put line 2431.


Package natbib Warning: Citation `Taylor_2000_SIAM' on page 112 undefined on in
put line 2436.


Package natbib Warning: Citation `Luo_2006_Luo' on page 112 undefined on input 
line 2436.


Package natbib Warning: Citation `karniadakis2005spectral' on page 112 undefine
d on input line 2436.

[112] [113] [114]

LaTeX Warning: Reference `eq: mapping' on page 115 undefined on input line 2505
.


LaTeX Warning: Reference `eq: NS_EQ_3D' on page 115 undefined on input line 250
9.


Package natbib Warning: Citation `Landmann_2010_AIAA' on page 115 undefined on 
input line 2509.


LaTeX Warning: Reference `fig: HEXA_FLUX' on page 115 undefined on input line 2
526.


LaTeX Warning: Reference `fig: HEXA_FLUX' on page 115 undefined on input line 2
526.


Package natbib Warning: Citation `kopriva1996conservative' on page 115 undefine
d on input line 2526.

[115 <./figures/mapping.pdf>]

LaTeX Warning: Reference `eq: Lagrange' on page 116 undefined on input line 253
5.

[116 <./figures/HEXA_FLUX_POINTS.pdf>]

Package natbib Warning: Citation `Toro_2013_Riemann' on page 117 undefined on i
nput line 2543.


Package natbib Warning: Citation `ruuth2006global' on page 117 undefined on inp
ut line 2543.


Package natbib Warning: Citation `Kopriva_1996_Mortar' on page 117 undefined on
 input line 2546.


LaTeX Warning: Reference `fig: Mortar' on page 117 undefined on input line 2548
.

[117]

Package natbib Warning: Citation `Kopriva_1996_Mortar' on page 118 undefined on
 input line 2560.


Package natbib Warning: Citation `Kopriva_1996_Mortar' on page 118 undefined on
 input line 2564.


LaTeX Warning: Reference `eq: MortarLeastSquare' on page 118 undefined on input
 line 2571.


LaTeX Warning: Reference `eq: MortarLeastSquare' on page 118 undefined on input
 line 2571.

[118 <./figures/Mortar.pdf>]

Package natbib Warning: Citation `KawaiLele_2008_JCP' on page 119 undefined on 
input line 2573.


Package natbib Warning: Citation `Premasuthan_2014_I' on page 119 undefined on 
input line 2573.


Package natbib Warning: Citation `Premasuthan_2014_II' on page 119 undefined on
 input line 2573.


LaTeX Warning: Reference `eq: stress_tensor' on page 119 undefined on input lin
e 2580.


LaTeX Warning: Reference `eq: heat_flux' on page 119 undefined on input line 25
80.

[119]

Package natbib Warning: Citation `SOD_1978_JCP' on page 120 undefined on input 
line 2609.


LaTeX Warning: Reference `fig: SOD_p' on page 120 undefined on input line 2609.



LaTeX Warning: Reference `fig: SOD_p_u' on page 120 undefined on input line 261
5.


Overfull \hbox (2.16397pt too wide) in paragraph at lines 2609--2616
\T1/cmr/m/n/12 men-sion-less left and right states de-fined as, $[]$ = $[]$ and
 $[] \OT1/cmr/m/n/12 =
[120 <./figures/1D_SOD_PAMR.pdf>]

Package natbib Warning: Citation `Jiang_1996_WENO' on page 121 undefined on inp
ut line 2628.


LaTeX Warning: Reference `eq: isentropicVortex' on page 121 undefined on input 
line 2634.


LaTeX Warning: Reference `eq: isentropicVortex' on page 121 undefined on input 
line 2634.


LaTeX Warning: Reference `fig: IsentropicVortex' on page 121 undefined on input
 line 2637.


LaTeX Warning: Reference `fig: IsentropicVortex' on page 121 undefined on input
 line 2637.


LaTeX Warning: Reference `eq: ShockSensor' on page 121 undefined on input line 
2641.


LaTeX Warning: Reference `eq: VorticitySensor' on page 121 undefined on input l
ine 2641.


LaTeX Warning: Reference `eq: ShockSensor' on page 121 undefined on input line 
2641.


LaTeX Warning: Reference `eq: VorticitySensor' on page 121 undefined on input l
ine 2641.

[121 <./figures/SOD_PAMR.pdf>]

LaTeX Warning: Reference `fig: VortexShockInteraction' on page 122 undefined on
 input line 2645.

[122 <./figures/VortexConvection.pdf>] [123 <./figures/vortex_shock_interaction
.pdf>] [124]
Chapter 8.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2657.

[125] [126]

Package natbib Warning: Citation `Lele_AnnRev_1994' on page 127 undefined on in
put line 2688.


Overfull \hbox (17.89577pt too wide) in paragraph at lines 2692--2693
[]\T1/cmr/m/n/12 Three regimes of ther-moa-cous-tic wave am-pli-fi-ca-tion were
 iden-ti-fied: ($\OML/cmm/m/it/12 i$\T1/cmr/m/n/12 ) a monochro-
[127]

Package natbib Warning: Citation `BsinghEtAl_2019_AIAA' on page 128 undefined o
n input line 2700.

[128]
Chapter 9.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2708.

[129] [130]
Chapter 10.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2880.


LaTeX Warning: Reference `eq: PressureMach' on page 131 undefined on input line
 2895.

[131pdfTeX warning (ext4): destination with the same identifier (name{equation.
10.0.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2910 \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.10.0.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2910 \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.10.0.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2910 \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.10.0.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2910 \end{align}
                  pdfTeX warning (ext4): destination with the same identifier (
name{equation.10.0.3}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.2910 \end{align}
                  ]

LaTeX Warning: Reference `eq: PressureStep1' on page 132 undefined on input lin
e 2911.


LaTeX Warning: Reference `eq: NS_eqns3' on page 132 undefined on input line 291
7.


LaTeX Warning: Reference `eq: per_norm_APP' on page 132 undefined on input line
 2917.


LaTeX Warning: Reference `eq: PressureStepAPP1' on page 132 undefined on input 
line 2922.


LaTeX Warning: Reference `eq: per_norm_APP' on page 132 undefined on input line
 2928.


LaTeX Warning: Reference `eq: PressureStepAPP2' on page 132 undefined on input 
line 2928.


LaTeX Warning: Reference `sec: 2ndOrderEntropy' on page 132 undefined on input 
line 2934.


LaTeX Warning: Reference `eq: NonDimEnt' on page 132 undefined on input line 29
34.


LaTeX Warning: Reference `eq: PressureStepAPP3' on page 132 undefined on input 
line 2934.

[132]

LaTeX Warning: Reference `eq: per_norm_APP' on page 133 undefined on input line
 2941.


LaTeX Warning: Reference `eq: NS_eqns2' on page 133 undefined on input line 294
1.


LaTeX Warning: Reference `eq: PressureStepAPP4' on page 133 undefined on input 
line 2946.


LaTeX Warning: Reference `eq: velocityStep1' on page 133 undefined on input lin
e 2946.


Underfull \hbox (badness 10000) in paragraph at lines 2945--2947


LaTeX Warning: Reference `eq: PressureStepAPP4' on page 133 undefined on input 
line 2948.


LaTeX Warning: Reference `eq: velocityStep1' on page 133 undefined on input lin
e 2948.


LaTeX Warning: Reference `eq: pressure' on page 133 undefined on input line 294
8.


LaTeX Warning: Reference `eq: velocity' on page 133 undefined on input line 294
8.


LaTeX Warning: Reference `eq: PressureStepAPP4' on page 133 undefined on input 
line 2957.


LaTeX Warning: Reference `eq: velocityStep1' on page 133 undefined on input lin
e 2957.


LaTeX Warning: Reference `eq: pressureAPP' on page 133 undefined on input line 
2957.


LaTeX Warning: Reference `eq: velocityAPP' on page 133 undefined on input line 
2957.


LaTeX Warning: Reference `sec: EnergyCorollary' on page 133 undefined on input 
line 2957.


LaTeX Warning: Reference `eq: Energy_norm' on page 133 undefined on input line 
2957.

[133] [134]
Chapter 11.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2960.


LaTeX Warning: Reference `eq: spectral_conservation' on page 135 undefined on i
nput line 2962.


LaTeX Warning: Reference `eq: pressure' on page 135 undefined on input line 296
2.


LaTeX Warning: Reference `eq: velocity' on page 135 undefined on input line 296
2.


LaTeX Warning: Reference `eq: p_spectral' on page 135 undefined on input line 2
971.


LaTeX Warning: Reference `eq: u_spectral' on page 135 undefined on input line 2
971.


LaTeX Warning: Reference `eq: pressure' on page 135 undefined on input line 297
8.

[135]

LaTeX Warning: Reference `eq: LinEq1' on page 136 undefined on input line 2983.



LaTeX Warning: Reference `eq: LinEq1' on page 136 undefined on input line 2995.



LaTeX Warning: Reference `eq: spectral_conservation' on page 136 undefined on i
nput line 2995.

[136]
Chapter 12.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 2998.


LaTeX Warning: Reference `sec: Linear' on page 137 undefined on input line 3005
.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 137 undefined
 on input line 3005.


Package natbib Warning: Citation `BiwaTY_JAcousSocAm_2011' on page 137 undefine
d on input line 3005.


Package natbib Warning: Citation `guedra_use_2012' on page 137 undefined on inp
ut line 3005.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 137 undefined
 on input line 3005.


LaTeX Warning: Reference `sec: Linear' on page 137 undefined on input line 3005
.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 137 undefined
 on input line 3005.


Package natbib Warning: Citation `BiwaTY_JAcousSocAm_2011' on page 137 undefine
d on input line 3005.


Package natbib Warning: Citation `guedra_use_2012' on page 137 undefined on inp
ut line 3005.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 137 undefined
 on input line 3005.


LaTeX Warning: Reference `fig: ExpValid' on page 137 undefined on input line 30
08.


LaTeX Warning: Reference `sec: Linear' on page 137 undefined on input line 3008
.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 137 undefined
 on input line 3008.


Package natbib Warning: Citation `guedra_use_2012' on page 137 undefined on inp
ut line 3008.


LaTeX Warning: Reference `fig:computational_setup' on page 137 undefined on inp
ut line 3008.


Package natbib Warning: Citation `Yazaki_PhysRevLet_1998' on page 137 undefined
 on input line 3008.


Package natbib Warning: Citation `guedra_use_2012' on page 137 undefined on inp
ut line 3008.


Package natbib Warning: Citation `BiwaTY_JAcousSocAm_2011' on page 137 undefine
d on input line 3009.


Package natbib Warning: Citation `BiwaEtAl_JASA_2014' on page 137 undefined on 
input line 3009.

[137 <./figures/Comparison.pdf>] [138]
Chapter 13.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 3012.


Overfull \hbox (7.87427pt too wide) detected at line 3032
[]

LaTeX Warning: Reference `eq: app_mom' on page 139 undefined on input line 3035
.


LaTeX Warning: Reference `eq: app_ent' on page 139 undefined on input line 3035
.

[139pdfTeX warning (ext4): destination with the same identifier (name{equation.
13.0.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.3}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.3036 \begin{eqnarray}
                       ]pdfTeX warning (ext4): destination with the same identi
fier (name{equation.13.0.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3036 \begin{eqnarray}
                       pdfTeX warning (ext4): destination with the same identif
ier (name{equation.13.0.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3054 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.13.0.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3054 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.13.0.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3054 \end{gather}
                    [140]
Chapter 14.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 3058.


LaTeX Warning: Reference `eq: 2_massApp' on page 141 undefined on input line 30
60.


LaTeX Warning: Reference `eq: 2_entApp' on page 141 undefined on input line 306
0.


LaTeX Warning: Reference `eq: ConstitutiveApp' on page 141 undefined on input l
ine 3081.


LaTeX Warning: Reference `eq: ContApp' on page 141 undefined on input line 3081
.


LaTeX Warning: Reference `eq: EntApp' on page 141 undefined on input line 3081.


[141]pdfTeX warning (ext4): destination with the same identifier (name{equation
.14.0.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3097 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.14.0.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3097 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.14.0.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3097 \end{gather}
                   pdfTeX warning (ext4): destination with the same identifier 
(name{equation.14.0.4}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.3097 \end{gather}
                   

LaTeX Warning: Reference `eq: nonlinear_P_App' on page 142 undefined on input l
ine 3100.


LaTeX Warning: Reference `eq: nonlinearities_App' on page 142 undefined on inpu
t line 3100.


LaTeX Warning: Reference `eq: u_modes' on page 142 undefined on input line 3102
.


LaTeX Warning: Reference `eq: s_modes' on page 142 undefined on input line 3102
.

[142]

LaTeX Warning: Reference `eq: shear_conv1' on page 143 undefined on input line 
3107.


LaTeX Warning: Reference `eq: heat_conv1' on page 143 undefined on input line 3
107.


LaTeX Warning: Reference `eq: analytical_un' on page 143 undefined on input lin
e 3111.


LaTeX Warning: Reference `eq: analytical_sn' on page 143 undefined on input lin
e 3111.


LaTeX Warning: Reference `eq: analytical_un' on page 143 undefined on input lin
e 3115.


LaTeX Warning: Reference `eq: analytical_sn' on page 143 undefined on input lin
e 3115.


LaTeX Warning: Reference `eq: approx_kernel' on page 143 undefined on input lin
e 3115.


Overfull \hbox (1.12048pt too wide) in paragraph at lines 3114--3116
\T1/cmr/m/n/12 for some func-tion $\OML/cmm/m/it/12 ^^^\OT1/cmr/m/n/12 (\OML/cm
m/m/it/12 x; t\OT1/cmr/m/n/12 )$\T1/cmr/m/n/12 . Af-ter sub-sti-tut-ing the abo
ve ap-prox-i-ma-tion in [] and [],
[143]
Chapter 15.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\uppercase' on input line 3117.


Package natbib Warning: Citation `persson:06' on page 144 undefined on input li
ne 3119.

[144] (./thesis.bbl [145] [146] [147] [148] [149] [150] [151] [152] [153]
[154] [155] [156])

Package natbib Warning: There were undefined citations.

[157] (./thesis.aux

Package natbib Warning: Citation(s) may have changed.
(natbib)                Rerun to get citations correct.


! Package natbib Error: Bibliography not compatible with author-year citations.

(natbib)                Press <return> to continue in numerical citation style.


See the natbib package documentation for explanation.
Type  H <return>  for immediate help.
 ...                                              
                                                  
l.794 ...and\NAT@force@numbers{}\NAT@force@numbers
                                                  
? Type <return> to proceed, S to scroll future error messages,
R to run without stopping, Q to run quietly,
I to insert something, E to edit your file,
1 or ... or 9 to ignore the next 1 to 9 tokens of input,
H for help, X to quit.
? 
! Emergency stop.
 ...                                              
                                                  
l.794 ...and\NAT@force@numbers{}\NAT@force@numbers
                                                  
!  ==> Fatal error occurred, no output PDF file produced!
Transcript written on thesis.log.


==> recommendations.tex <==
%
%  recommendations.tex  2007-02-06  Mark Senn  http://www.ecn.purdue.edu/~mark
%

\chapter{Recommendations}

Buy low.  Sell high.


==> vita.tex <==
%
%  vita.tex   2003.07.23  14:59:33   Mark Senn <mds@purdue.edu>
%
%  This is the vita for a simple, example thesis.
%
%  A vita is required only in a doctoral dissertation.
%

\begin{vita}
    [Put a brief autobiographical sketch here.]
\end{vita}

